The phonetic bases of vocal expressed emotion: natural versus acted

Can vocal emotions be emulated? This question has been a recurrent concern of the speech community, and has also been vigorously investigated. It has been fueled further by its link to the issue of validity of acted emotion databases. Much of the speech and vocal emotion research has relied on acted emotion databases as valid proxies for studying natural emotions. To create models that generalize to natural settings, it is crucial to work with valid prototypes -- ones that can be assumed to reliably represent natural emotions. More concretely, it is important to study emulated emotions against natural emotions in terms of their physiological, and psychological concomitants. In this paper, we present an on-scale systematic study of the differences between natural and acted vocal emotions. We use a self-attention based emotion classification model to understand the phonetic bases of emotions by discovering the most 'attended' phonemes for each class of emotions. We then compare these attended-phonemes in their importance and distribution across acted and natural classes. Our tests show significant differences in the manner and choice of phonemes in acted and natural speech, concluding moderate to low validity and value in using acted speech databases for emotion classification tasks.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> LaTeX/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> LaTeX/intro2.tex <==

\section{Introduction}
\label{sec:intro}
\emph{Can vocal emotions be emulated?}  This question has led to long standing debates in the speech community regarding \emph{natural} versus \emph{acted} emotions, in the context of emotion classification and emotion categorization tasks. 
To conduct any speech based emotion research, an important factor is the nature of the speech samples or the vocal stimuli, and whether those samples are representative of natural emotions. 
Natural emotions can best be defined as emotions that are spontaneous and involuntary. Acted emotions, on the other hand, are prompted and voluntary. 
Because acted emotions are volitional, researchers argue that the physiological and psychological responses that natural emotions induce are absent from acted emotions
 \cite{jurgens2015effect,wilting2006real}. Nevertheless, research on emotion perception uses acted emotions as convenient proxies for natural emotions. While many past studies have focused on presenting perception tests for natural versus acted emotions with mixed conclusions \cite{wilting2006real,scherer2013vocal,audibert2008we}, there is a lack of an at-scale systematic framework to study the differences and similarities in those classes. 

There are, in fact, two facets to vocally expressed emotion: emotion, as it is {\em experienced} by the speaker, which is a total-body phenomenon involving physiological and psychological changes, and  emotion, as it is {\em perceived} by the listener, who then interprets it to implicitly infer the underlying state of the speaker. The job of the actor is to produce speech that creates the same impression in the listener vis-a-vis the emotional state of the speaker, as naturally expressed emotion.

\begin{figure}[htb]
  \centering
   \centerline{\includegraphics[width=6cm]{Images/noa_model.png}}
%  \vspace{1.5cm}
%   \centerline{Phoneme distribution}\medskip
  \caption{The non-actor, actor and observer (NAO) framework for the communication of emotions.}
    \label{fig:noa_model}
\end{figure}
% In this paper, we present a novel framework to study natural and acted vocal emotions.
% in the context of their \emph{phonetic bases}. 

To elaborate on the distinction between the three, we use our proposed \emph{non-actor, actor, and observer (NAO)} framework as shown in figure \ref{fig:noa_model}. 
The communication of vocal emotions is primarily a combination of an encoding and a decoding process. The subject {\em expressing} the emotion encodes their emotional state into the low-dimensional speech signal. The subject {\em perceiving} the signal decodes it to make inferences about the state of being of the speaker. 
We will distinguish between two types of encoders:  the {\em non-actor} who actually experiences the emotion, and the {\em actor} who may not. In all cases, the decoder is an {\em observer}, who's only cue in terms of vocal emotions is the vocal stimuli. 
%%%From an evolutionary perspective, an observer is primarily cognizant of natural emotions and their cues. 
%%5Encoding of emotions, on the other hand, can differ between natural and acted classes. Because natural emotions are, for the most part, involuntary, they include physiological and psychological responses as concomitants. 
%%%These emotions may or may not have an intended audience. On the other hand, acted emotions are intended for an audience. 
The job of the \emph{actor} here is to emulate the natural emotions (of the non-actors) such that the observer is not able to differentiate between natural and acted stimuli, and may somewhat be deceived. 
%In some sense, our NAO model is a test for real versus acted emotions. 
% The question th test passes, however, that would signal towards dichotomy between acted and natural emotions, leading to a low validity and value in using acted stimuli.

%The vocal encodingen is whether the observer is able to tell apart natural emotions from acted emotions based on some of the features of the vocal stimuli.
% in which case the test passes, else the test fails. 
% If the test fails, that would mean natural emotions \emph{can} be emulated, and that acted emotions can be used as proxies for natural emotions. 


%In some sense, our NAO model is a test for real versus acted emotions. The question then is whether we are able to tell apart natural emotions from acted emotions based on some of the features of the vocal stimuli, in which case the test passes, else the test fails. If the test fails, that would mean natural emotions \emph{can} be emulated, and that acted emotions can be used as proxies for natural emotions. If the test passes, however, that would signal towards dichotomy between acted and natural emotions, leading to a low validity and value in using acted stimuli.

We note that encoding of emotions can differ between natural and acted classes. Because natural emotions are, for the most part, involuntary, they include physiological and psychological responses as concomitants, such as heart rate, breathing rate, muscle tension, and mood. The physiological changes manifest in the voice by changing the spectro-temporal structure of individual sounds \cite{johnstone1999effects, scherer1977cue}. For example, \cite{williams1972emotions, myers2013inherent} argue that vowels and consonants produced in \emph{fear} are often more precisely articulated than they are in \emph{neutral} situations. The physiological changes along with the psychological factors also define the choice of phonemes (i.e. the lexical content). As an example, words of aggressive nature are more likely to be used by an individual in an aggressive mood \cite{whissell1999phonosymbolism}. 

In sum, natural emotion results in concomitant-induced changes to many facets of the speech signal. The observer perceives an {\em aggregate} of these changes to make their inference about the emotional state of the speaker. In emulating an emotion, the actor attempts to (and may even succeed) in producing the same {\em aggregate} of these factors as the non-actor. We hypothesize that in doing so,  the {\em individual factors} that the actor produces will, however, be implausible, and easily distinguished, though the human observer may not do so in a natural setting. I.e. even if an observer is fooled (e.g. by a very skilled actor), the signal itself is useless as an indicator of the natural state of the actor, leading to a low validity and value in using acted stimuli in paralinguistic analysis of speech.


%Vocal communication of emotion constitutes of various factors, like prosodic cues, phonetic distribution and phonetic emphasis. We hypothesize that although the natural expression of vocal emotion constitutes of these factors, the acted expression misses some factors or does not capture them correctly. An actor can combine a good facsimile of these factors to emulate natural speech, but the individual components will be implausible. To achieve this, the actor will emulate some indistinguishable combination of vocal stimuli factors. However, even in doing so, the individual components will not be captured correctly. 

To explain this point, we take the help of an Oliver Sacks case study ``The President's Speech'' \cite{sacks1985president} in which  there are two types of patients: \emph{aphasic}, and \emph{tonal agnostic}. \emph{Aphasic} patients are highly sensitive to expression and tone, and focus on the expressiveness of the emotion to capture it. On the other hand, \emph{tonal agnostic} patients lack any sense of expression and tone, and pay attention to exactness of words and word use to capture the emotion. Neither of these patients can grasp the totality of the natural emotion. However, unlike normal people, these patients, both aphasic and tonal agnostic, can not be lied to or deceived as they have the ability to focus on certain individual factors of emotion which can not be substituted for factors in natural emotion. 

% IT GOES SOUTH FROM HERE.  THE STUFF BELOW HAS NO RELATION TO THE STUFF ABOVE




% Therefore, in this study, we try to model the observer in the NAO model. The focus is on what part of the vocal stimuli does the observer \emph{attend} to in order to determine the vocal emotion. 
%These factors are a result of physiological and psychological changes in the speaker such as the heart rate, breathing rate, muscle tension, and mood. The physiological changes manifest in the voice by changing the spectro-temporal structure of individual sounds \cite{johnstone1999effects, scherer1977cue}. For example, \cite{williams1972emotions, myers2013inherent} argue that vowels and consonants produced in \emph{fear} are often more precisely articulated than they are in \emph{neutral} situations. The physiological changes along with the psychological factors also define the choice of phonemes (i.e. the lexical content). As an example, words of aggressive nature are more likely to be used by an individual in an aggressive mood \cite{whissell1999phonosymbolism}. 

We identify two (of the many) basic factors of vocally-expressed emotion, \emph{choice of phonemes} and their \emph{manner of delivery}, which we call the \emph{phonetic bases of vocal emotions}. 
%
% we investigate the phonetic bases of vocal emotions. We define phonetic bases as the \emph{choice of phonemes} and their \emph{manner of delivery}. These phonetic bases are a result of 
By our hypothesis, these phonetic bases are different in natural and acted emotions.  

To verify our hypothesis, we require a mechanism to tease apart these bases from the speech signal. We train a neural network model for emotion classification tasks on two datasets using \emph{attention} mechanism. The attention aims to capture the phonetic bases of an utterance in order to classify for emotion. We quantify the most \emph{attentive} phonemes under two datasets and compare them across the emotions. As we will see in the final sections of our paper, these factors do indeed differ in a statisically significant manner.

% Unlike a traditional lab setting with controlled variables, we conduct an uncontrolled post-hoc analyses over two existing databases with different speakers and content. To ensure that our analyses have no confounding variables, we, therefore, conduct experimental validation tests to control for any speaker and content-specific biases in databases. 

% \vspace{-1em}



==> LaTeX/intro3.tex <==

\section{Introduction}
\label{sec:intro}
\emph{Can vocal emotions be emulated?}  This question has led to long standing debates in the speech community regarding \emph{natural} versus \emph{acted} emotions, in the context of emotion classification and emotion categorization tasks. 
To conduct any speech based emotion research, an important factor is the nature of the speech samples or the vocal stimuli, and whether those samples are representative of natural emotions. 
Natural emotions can best be defined as emotions that are spontaneous and involuntary. Acted emotions, on the other hand, are prompted and voluntary. 
Because acted emotions are volitional, researchers argue that the physiological and psychological responses that natural emotions induce are absent from acted emotions
 \cite{jurgens2015effect,wilting2006real}. Nevertheless, research on emotion perception uses acted emotions as convenient proxies for natural emotions. While many past studies have focused on presenting perception tests for natural versus acted emotions with mixed conclusions \cite{wilting2006real,scherer2013vocal,audibert2008we}, there is a lack of an at-scale systematic framework to study the differences and similarities in those classes. 

In order to develop such a framework, we must recognize that there are, in fact {\em three entities} to be considered.
The communication of vocal emotions is, at its essence, a combination of an encoding and a decoding process. The subject {\em expressing} the emotion encodes their emotional state into the low-dimensional speech signal. The subject {\em perceiving} the signal decodes it to make inferences about the state of the speaker. We will distinguish between two types of encoders:  the {\em non-actor} who actually experiences the emotion, and the {\em actor} who may not. In all cases, the decoder is an {\em observer}, who's only cue in terms of vocal emotions is the vocal stimuli. Based on these, we propose the \emph{non-actor, actor, and observer (NAO)} model (Figure \ref{fig:noa_model}), which represents all three entities and the relation between them. The actor aims to encode synthetic emotion in a manner that the observer cannot distinguish from the genuine emotion encoded by the non-actor. This enables us to formulate a hypothesis that can be formally tested -- that there nevertheless remain identifiable fundamental differences in the encoded signals in the two cases. If the test fails, that would mean natural emotions \emph{can} be emulated, and that acted emotions can be used as proxies for natural emotions. If the test passes, however, that would signal towards dichotomy between acted and natural emotions, leading to a low validity and value in using acted stimuli.


% To  we use our proposed \emph{non-actor, actor, and observer (NAO)} framework as shown in figure \ref{fig:noa_model}.

\begin{figure}[htb]
  \centering
   \centerline{\includegraphics[width=6cm]{Images/noa_model.png}}
%  \vspace{1.5cm}
%   \centerline{Phoneme distribution}\medskip
  \caption{The non-actor, actor and observer (NAO) framework for the communication of emotions.}
    \label{fig:noa_model}
\end{figure}

We note that non-actor and the actor differ in their encoding of emotions. Because natural emotions are, for the most part, involuntary, they include physiological and psychological responses as concomitants, such as heart rate, breathing rate, muscle tension, and mood. These physiological changes manifest in the voice by changing the spectro-temporal structure of individual sounds \cite{johnstone1999effects, scherer1977cue}. For example, \cite{williams1972emotions, myers2013inherent} argue that vowels and consonants produced in \emph{fear} are often more precisely articulated than they are in \emph{neutral} situations. The physiological changes along with the psychological factors also define the choice of phonemes (i.e. the lexical content) and prosodic cues \cite{scherer2003vocal, patel2011mapping}. As an example, words of aggressive nature are more likely to be used by an individual in an aggressive mood \cite{whissell1999phonosymbolism}. 
% [STATEMENT ABOUT HOW THE ENCODING OF EMOTION IS ACTUALLY THROUGH THE AGGREGATE OF THESE FACTORS]
% In sum, natural emotion results in concomitant-induced changes to many facets of the speech signal. 
The  encoding of emotion is hence an aggregate, or {\em perceptual sum} of these acoustic, phonetic and linguistic influences, or {\em factors}. 
The observer decodes the perceptual sum of these factors to make their inference about the emotional state of the speaker. 


% [THIS CAN MOVE]On the other hand, the actor does not experience these [NATURA?]changes.  %% GOES and has to rely on his imitation skills in an attempt to express an emotion.  



In emulating an emotion, the actor attempts to produce a somewhat similar {\em aggregate} of these factors as the non-actor, {\em i.e.} a combination of factors that he expects the observer to decode into a near identical perceptual sum. If the actor succeeds, he conveys the target emotion to the observer. We hypothesize that in doing so,  the {\em individual factors} that the actor produces will, however, still be incorrect or even implausible, even though the perceptual sum may be plausible. 
%One of the most implausible of these factors are a result of physiological and psychological changes in the speaker, because the actor does not experience these changes.
% I.e. even if an observer is fooled (e.g. by a very skilled actor), the signal itself is useless as an indicator of the natural state of the actor, leading to a low validity and value in using acted stimuli in paralinguistic analysis of speech.


%Vocal communication of emotion constitutes of various factors, like prosodic cues, phonetic distribution and phonetic emphasis. We hypothesize that although the natural expression of vocal emotion constitutes of these factors, the acted expression misses some factors or does not capture them correctly. An actor can combine a good facsimile of these factors to emulate natural speech, but the individual components will be implausible. To achieve this, the actor will emulate some indistinguishable combination of vocal stimuli factors. However, even in doing so, the individual components will not be captured correctly. 

% [THE INDIVIDUALITY OF THESE FACTORS IS BEST ILLUSTRATED BY A CASE STUDY BY THE FAMOUS OLIVER SACKS:  THE ...]
The distinction is, perhaps,  best illustrated by the study, ``The President's Speech'', narrated by well-known neurologist Oliver Sacks  \cite{sacks1985president}, in which two types of patients, \emph{aphasic}, and \emph{tonal agnostic}, both find a presidential candidate's posturing on TV to be screamingly implausible, although normal viewers have no problem with it. \emph{Aphasic} patients are highly sensitive to expression and tone, but cannot interpret the words. On the other hand, \emph{tonal agnostic} patients lack any sense of expression and tone, and pay attention to exactness of words and word use to capture the emotion. The skilled actor, in this case the presidential candidate, attempts to convey feelings and emotions through a combination of affect that is given a pass by normal viewers.
%Neither of these patients can grasp the totality of the natural emotion. 
However, both types of patients who, unlike normal people, only perceive some of these factors, find them sufficiently implausible as to cause them distress. Simply by their inability to consider the totality of affect that normal people can perceive, the patients cannot be lied to or deceived.
% as they have the ability to focus on certain individual factors of emotion which can not be substituted for factors in natural emotion. 

% IT GOES SOUTH FROM HERE.  THE STUFF BELOW HAS NO RELATION TO THE STUFF ABOVE


% Therefore, in this study, we try to model the observer in the NAO model. The focus is on what part of the vocal stimuli does the observer \emph{attend} to in order to determine the vocal emotion. 
%These factors are a result of physiological and psychological changes in the speaker such as the heart rate, breathing rate, muscle tension, and mood. The physiological changes manifest in the voice by changing the spectro-temporal structure of individual sounds \cite{johnstone1999effects, scherer1977cue}. For example, \cite{williams1972emotions, myers2013inherent} argue that vowels and consonants produced in \emph{fear} are often more precisely articulated than they are in \emph{neutral} situations. The physiological changes along with the psychological factors also define the choice of phonemes (i.e. the lexical content). As an example, words of aggressive nature are more likely to be used by an individual in an aggressive mood \cite{whissell1999phonosymbolism}. 

Vocal (or indeed any) expression of emotion is, of course, a complex phenomenon, and the complete set of acoustic, phonetic, linguistic and prosodic factors used in expressing it is still not fully understood. To test our hypothesis, we must nevertheless identify one or more of these factors that can be statistically quantified. As mentioned earlier, physiological and psychological changes concomitant with emotion are known to affect the \emph{choice of phonemes} and their \emph{manner of delivery}. We will refer to these as the \emph{phonetic bases of vocal emotions}. By our hypothesis, there will be a statistically measurable difference in these between the actor and non-actor.


To verify our hypothesis, we require a mechanism to quantiably extract these bases from the speech signal. To do so, we train a neural network model for emotion classification tasks on two datasets, one of natural speech and the other of acted emotional speech, using an \emph{attention} mechanism. The attention aims to identify the most important phonemes in an utterance in order to classify its  emotion. We compare the statistical patterns of the most \emph{attented} phonemes across actor and non-actor. As we will see in the final sections of our paper, these factors do indeed differ in a statistically significant manner, bringing the validity of conclusions drawn from acted emotional speech as a proxy for natural emotion into question.

. 

% Unlike a traditional lab setting with controlled variables, we conduct an uncontrolled post-hoc analyses over two existing databases with different speakers and content. To ensure that our analyses have no confounding variables, we, therefore, conduct experimental validation tests to control for any speaker and content-specific biases in databases. 

% \vspace{-1em}



==> LaTeX/old_intro.tex <==

\section{Introduction}
\label{sec:intro}
\emph{Can vocal emotions be emulated?}  This question has led to long standing debates in the speech community regarding \emph{natural} versus \emph{acted} emotions, in the context of emotion classification and emotion categorization tasks. 
To conduct any speech based emotion research, an important factor is the nature of the speech samples or the vocal stimuli, and whether those samples are representative of natural emotions. 
Natural emotions can best be defined as emotions that are spontaneous and involuntary. Acted emotions, on the other hand, are prompted and voluntary. 
Because acted emotions are volitional, researchers argue that the physiological and psychological responses that natural emotions induce are absent from acted emotions
 \cite{jurgens2015effect,wilting2006real}. Nevertheless, research on emotion perception uses acted emotions as convenient proxies for natural emotions. While many past studies have focused on presenting perception tests for natural versus acted emotions with mixed conclusions \cite{wilting2006real,scherer2013vocal,audibert2008we}, there is a lack of an at-scale systematic framework to study the differences and similarities in those classes. 

Vocal communication of emotion constitutes of various factors, like prosodic cues, phonetic distribution and phonetic emphasis. We hypothesize that although the natural expression of vocal emotion constitutes of these factors, the acted expression misses some factors or does not capture them correctly. An actor can combine a good facsimile of these factors to emulate natural speech, but the individual components will be implausible. 



\begin{figure}[htb]
  \centering
   \centerline{\includegraphics[width=6cm]{Images/noa_model.png}}
%  \vspace{1.5cm}
%   \centerline{Phoneme distribution}\medskip
  \caption{The non-actor, actor and observer (NAO) framework for the communication of emotions.}
    \label{fig:noa_model}
\end{figure}
% In this paper, we present a novel framework to study natural and acted vocal emotions.
% in the context of their \emph{phonetic bases}. 

To further elaborate, we use our proposed \emph{non-actor, actor, and observer (NAO)} framework as shown in figure \ref{fig:noa_model}. 
% The communication of vocal emotions is primarily based on its encoding and decoding process. Encoding of emotions is what we call an \emph{expression}, whereas the process of decoding is called \emph{perception}. 
 The subject decoding the emotions and hence perceiving them is an \emph{observer} whose only cue in terms of vocal emotions is the vocal stimuli. 
% From an evolutionary perspective, an observer is primarily cognizant of natural emotions and their cues. 
% Encoding of emotions, on the other hand, can differ between natural and acted classes. Because natural emotions are, for the most part, involuntary, they include physiological and psychological responses as concomitants. 
% These emotions may or may not have an intended audience. On the other hand, acted emotions are intended for an audience. 
The job of the \emph{actor} here is to emulate the natural emotions (of the non-actors) such that the observer is not able to differentiate between natural and acted stimuli, and may somewhat be deceived. To achieve this, the actor will emulate some indistinguishable combination of vocal stimuli factors. However, even in doing so, the individual components will not be captured correctly. 
To explain this point, we take the help of an Oliver Sacks case study ``The President's Speech'' \cite{sacks1985president} in which  there are two types of patients: \emph{aphasic}, and \emph{tonal agnostic}. \emph{Aphasic} patients are highly sensitive to expression and tone, and focus on the expressiveness of the emotion to capture it. On the other hand, \emph{tonal agnostic} patients lack any sense of expression and tone, and pay attention to exactness of words and word use to capture the emotion. Neither of these patients can grasp the totality of the natural emotion. However, unlike normal people, these patients, both aphasic and tonal agnostic, can not be lied to or deceived as they have the ability to focus on certain individual factors of emotion which can not be substituted for factors in natural emotion. 

% IT GOES SOUTH FROM HERE.  THE STUFF BELOW HAS NO RELATION TO THE STUFF ABOVE


% In some sense, our NAO model is a test for real versus acted emotions. 
% The question then is whether the observer is able to tell apart natural emotions from acted emotions based on some of the features of the vocal stimuli.
% in which case the test passes, else the test fails. 
% If the test fails, that would mean natural emotions \emph{can} be emulated, and that acted emotions can be used as proxies for natural emotions. If the test passes, however, that would signal towards dichotomy between acted and natural emotions, leading to a low validity and value in using acted stimuli.

% Therefore, in this study, we try to model the observer in the NAO model. The focus is on what part of the vocal stimuli does the observer \emph{attend} to in order to determine the vocal emotion. 
These factors are a result of physiological and psychological changes in the speaker such as the heart rate, breathing rate, muscle tension, and mood. The physiological changes manifest in the voice by changing the spectro-temporal structure of individual sounds \cite{johnstone1999effects, scherer1977cue}. For example, \cite{williams1972emotions, myers2013inherent} argue that vowels and consonants produced in \emph{fear} are often more precisely articulated than they are in \emph{neutral} situations. The physiological changes along with the psychological factors also define the choice of phonemes (i.e. the lexical content). As an example, words of aggressive nature are more likely to be used by an individual in an aggressive mood \cite{whissell1999phonosymbolism}. 
Following this, we determine two basic factors of emotion, \emph{choice of phonemes} and their \emph{manner of delivery}, which we call the \emph{phonetic bases of vocal emotions}. 

% we investigate the phonetic bases of vocal emotions. We define phonetic bases as the \emph{choice of phonemes} and their \emph{manner of delivery}. These phonetic bases are a result of 
Our hypothesis is that these phonetic bases are different in natural and acted emotions.
To test our hypothesis, we train a neural network model for emotion classification tasks on two datasets using \emph{attention} mechanism. The attention aims to capture the phonetic bases of an utterance in order to classify for emotion. We quantify the most \emph{attentive} phonemes under two datasets and compare them across the emotions.

% Unlike a traditional lab setting with controlled variables, we conduct an uncontrolled post-hoc analyses over two existing databases with different speakers and content. To ensure that our analyses have no confounding variables, we, therefore, conduct experimental validation tests to control for any speaker and content-specific biases in databases. 

% \vspace{-1em}


% The communication of vocal emotions which is primarily a combination of an encoding and a decoding process, can be elaborated through the NAO model. The subject {\em expressing} the emotion encodes their emotional state into the low-dimensional speech signal. The subject {\em perceiving} the signal decodes it to make inferences about the state of being of the speaker. We will distinguish between two types of encoders:  the {\em non-actor} who actually experiences the emotion, and the {\em actor} who may not. In all cases, the decoder is an {\em observer}, who's only cue in terms of vocal emotions is the vocal stimuli. The job of the \emph{actor} here is to emulate the natural emotions (of the non-actors) such that the observer is not able to differentiate between natural and acted stimuli, and may somewhat be deceived. 


==> intro2.tex <==

\section{Introduction}
\label{sec:intro}
\emph{Can vocal emotions be emulated?}  This question has led to long standing debates in the speech community regarding \emph{natural} versus \emph{acted} emotions, in the context of emotion classification and emotion categorization tasks. 
To conduct any speech based emotion research, an important factor is the nature of the speech samples or the vocal stimuli, and whether those samples are representative of natural emotions. 
Natural emotions can best be defined as emotions that are spontaneous and involuntary. Acted emotions, on the other hand, are prompted and voluntary. 
Because acted emotions are volitional, researchers argue that the physiological and psychological responses that natural emotions induce are absent from acted emotions
 \cite{jurgens2015effect,wilting2006real}. Nevertheless, research on emotion perception uses acted emotions as convenient proxies for natural emotions. While many past studies have focused on presenting perception tests for natural versus acted emotions with mixed conclusions \cite{wilting2006real,scherer2013vocal,audibert2008we}, there is a lack of an at-scale systematic framework to study the differences and similarities in those classes. 

There are, in fact, two facets to vocally expressed emotion: emotion, as it is {\em experienced} by the speaker, which is a total-body phenomenon involving physiological and psychological changes, and  emotion, as it is {\em perceived} by the listener, who then interprets it to implicitly infer the underlying state of the speaker. The job of the actor is to produce speech that creates the same impression in the listener vis-a-vis the emotional state of the speaker, as naturally expressed emotion.

\begin{figure}[htb]
  \centering
   \centerline{\includegraphics[width=6cm]{Images/noa_model.png}}
%  \vspace{1.5cm}
%   \centerline{Phoneme distribution}\medskip
  \caption{The non-actor, actor and observer (NAO) framework for the communication of emotions.}
    \label{fig:noa_model}
\end{figure}
% In this paper, we present a novel framework to study natural and acted vocal emotions.
% in the context of their \emph{phonetic bases}. 

To elaborate on the distinction between the three, we use our proposed \emph{non-actor, actor, and observer (NAO)} framework as shown in figure \ref{fig:noa_model}. 
The communication of vocal emotions is primarily a combination of an encoding and a decoding process. The subject {\em expressing} the emotion encodes their emotional state into the low-dimensional speech signal. The subject {\em perceiving} the signal decodes it to make inferences about the state of being of the speaker. 
We will distinguish between two types of encoders:  the {\em non-actor} who actually experiences the emotion, and the {\em actor} who may not. In all cases, the decoder is an {\em observer}, who's only cue in terms of vocal emotions is the vocal stimuli. 
%%%From an evolutionary perspective, an observer is primarily cognizant of natural emotions and their cues. 
%%5Encoding of emotions, on the other hand, can differ between natural and acted classes. Because natural emotions are, for the most part, involuntary, they include physiological and psychological responses as concomitants. 
%%%These emotions may or may not have an intended audience. On the other hand, acted emotions are intended for an audience. 
The job of the \emph{actor} here is to emulate the natural emotions (of the non-actors) such that the observer is not able to differentiate between natural and acted stimuli, and may somewhat be deceived. 
%In some sense, our NAO model is a test for real versus acted emotions. 
% The question th test passes, however, that would signal towards dichotomy between acted and natural emotions, leading to a low validity and value in using acted stimuli.

%The vocal encodingen is whether the observer is able to tell apart natural emotions from acted emotions based on some of the features of the vocal stimuli.
% in which case the test passes, else the test fails. 
% If the test fails, that would mean natural emotions \emph{can} be emulated, and that acted emotions can be used as proxies for natural emotions. 


%In some sense, our NAO model is a test for real versus acted emotions. The question then is whether we are able to tell apart natural emotions from acted emotions based on some of the features of the vocal stimuli, in which case the test passes, else the test fails. If the test fails, that would mean natural emotions \emph{can} be emulated, and that acted emotions can be used as proxies for natural emotions. If the test passes, however, that would signal towards dichotomy between acted and natural emotions, leading to a low validity and value in using acted stimuli.

We note that encoding of emotions can differ between natural and acted classes. Because natural emotions are, for the most part, involuntary, they include physiological and psychological responses as concomitants, such as heart rate, breathing rate, muscle tension, and mood. The physiological changes manifest in the voice by changing the spectro-temporal structure of individual sounds \cite{johnstone1999effects, scherer1977cue}. For example, \cite{williams1972emotions, myers2013inherent} argue that vowels and consonants produced in \emph{fear} are often more precisely articulated than they are in \emph{neutral} situations. The physiological changes along with the psychological factors also define the choice of phonemes (i.e. the lexical content). As an example, words of aggressive nature are more likely to be used by an individual in an aggressive mood \cite{whissell1999phonosymbolism}. 

In sum, natural emotion results in concomitant-induced changes to many facets of the speech signal. The observer perceives an {\em aggregate} of these changes to make their inference about the emotional state of the speaker. In emulating an emotion, the actor attempts to (and may even succeed) in producing the same {\em aggregate} of these factors as the non-actor. We hypothesize that in doing so,  the {\em individual factors} that the actor produces will, however, be implausible, and easily distinguished, though the human observer may not do so in a natural setting. I.e. even if an observer is fooled (e.g. by a very skilled actor), the signal itself is useless as an indicator of the natural state of the actor, leading to a low validity and value in using acted stimuli in paralinguistic analysis of speech.


%Vocal communication of emotion constitutes of various factors, like prosodic cues, phonetic distribution and phonetic emphasis. We hypothesize that although the natural expression of vocal emotion constitutes of these factors, the acted expression misses some factors or does not capture them correctly. An actor can combine a good facsimile of these factors to emulate natural speech, but the individual components will be implausible. To achieve this, the actor will emulate some indistinguishable combination of vocal stimuli factors. However, even in doing so, the individual components will not be captured correctly. 

To explain this point, we take the help of an Oliver Sacks case study ``The President's Speech'' \cite{sacks1985president} in which  there are two types of patients: \emph{aphasic}, and \emph{tonal agnostic}. \emph{Aphasic} patients are highly sensitive to expression and tone, and focus on the expressiveness of the emotion to capture it. On the other hand, \emph{tonal agnostic} patients lack any sense of expression and tone, and pay attention to exactness of words and word use to capture the emotion. Neither of these patients can grasp the totality of the natural emotion. However, unlike normal people, these patients, both aphasic and tonal agnostic, can not be lied to or deceived as they have the ability to focus on certain individual factors of emotion which can not be substituted for factors in natural emotion. 

% IT GOES SOUTH FROM HERE.  THE STUFF BELOW HAS NO RELATION TO THE STUFF ABOVE




% Therefore, in this study, we try to model the observer in the NAO model. The focus is on what part of the vocal stimuli does the observer \emph{attend} to in order to determine the vocal emotion. 
%These factors are a result of physiological and psychological changes in the speaker such as the heart rate, breathing rate, muscle tension, and mood. The physiological changes manifest in the voice by changing the spectro-temporal structure of individual sounds \cite{johnstone1999effects, scherer1977cue}. For example, \cite{williams1972emotions, myers2013inherent} argue that vowels and consonants produced in \emph{fear} are often more precisely articulated than they are in \emph{neutral} situations. The physiological changes along with the psychological factors also define the choice of phonemes (i.e. the lexical content). As an example, words of aggressive nature are more likely to be used by an individual in an aggressive mood \cite{whissell1999phonosymbolism}. 

We identify two (of the many) basic factors of vocally-expressed emotion, \emph{choice of phonemes} and their \emph{manner of delivery}, which we call the \emph{phonetic bases of vocal emotions}. 
%
% we investigate the phonetic bases of vocal emotions. We define phonetic bases as the \emph{choice of phonemes} and their \emph{manner of delivery}. These phonetic bases are a result of 
By our hypothesis, these phonetic bases are different in natural and acted emotions.  

To verify our hypothesis, we require a mechanism to tease apart these bases from the speech signal. We train a neural network model for emotion classification tasks on two datasets using \emph{attention} mechanism. The attention aims to capture the phonetic bases of an utterance in order to classify for emotion. We quantify the most \emph{attentive} phonemes under two datasets and compare them across the emotions. As we will see in the final sections of our paper, these factors do indeed differ in a statisically significant manner.

% Unlike a traditional lab setting with controlled variables, we conduct an uncontrolled post-hoc analyses over two existing databases with different speakers and content. To ensure that our analyses have no confounding variables, we, therefore, conduct experimental validation tests to control for any speaker and content-specific biases in databases. 

% \vspace{-1em}



==> old_intro.tex <==

\section{Introduction}
\label{sec:intro}
\emph{Can vocal emotions be emulated?}  This question has led to long standing debates in the speech community regarding \emph{natural} versus \emph{acted} emotions, in the context of emotion classification and emotion categorization tasks. 
To conduct any speech based emotion research, an important factor is the nature of the speech samples or the vocal stimuli, and whether those samples are representative of natural emotions. 
Natural emotions can best be defined as emotions that are spontaneous and involuntary. Acted emotions, on the other hand, are prompted and voluntary. 
Because acted emotions are volitional, researchers argue that the physiological and psychological responses that natural emotions induce are absent from acted emotions
 \cite{jurgens2015effect,wilting2006real}. Nevertheless, research on emotion perception uses acted emotions as convenient proxies for natural emotions. While many past studies have focused on presenting perception tests for natural versus acted emotions with mixed conclusions \cite{wilting2006real,scherer2013vocal,audibert2008we}, there is a lack of an at-scale systematic framework to study the differences and similarities in those classes. 

Vocal communication of emotion constitutes of various factors, like prosodic cues, phonetic distribution and phonetic emphasis. We hypothesize that although the natural expression of vocal emotion constitutes of these factors, the acted expression misses some factors or does not capture them correctly. An actor can combine a good facsimile of these factors to emulate natural speech, but the individual components will be implausible. 



\begin{figure}[htb]
  \centering
   \centerline{\includegraphics[width=6cm]{Images/noa_model.png}}
%  \vspace{1.5cm}
%   \centerline{Phoneme distribution}\medskip
  \caption{The non-actor, actor and observer (NAO) framework for the communication of emotions.}
    \label{fig:noa_model}
\end{figure}
% In this paper, we present a novel framework to study natural and acted vocal emotions.
% in the context of their \emph{phonetic bases}. 

To further elaborate, we use our proposed \emph{non-actor, actor, and observer (NAO)} framework as shown in figure \ref{fig:noa_model}. 
% The communication of vocal emotions is primarily based on its encoding and decoding process. Encoding of emotions is what we call an \emph{expression}, whereas the process of decoding is called \emph{perception}. 
 The subject decoding the emotions and hence perceiving them is an \emph{observer} whose only cue in terms of vocal emotions is the vocal stimuli. 
% From an evolutionary perspective, an observer is primarily cognizant of natural emotions and their cues. 
% Encoding of emotions, on the other hand, can differ between natural and acted classes. Because natural emotions are, for the most part, involuntary, they include physiological and psychological responses as concomitants. 
% These emotions may or may not have an intended audience. On the other hand, acted emotions are intended for an audience. 
The job of the \emph{actor} here is to emulate the natural emotions (of the non-actors) such that the observer is not able to differentiate between natural and acted stimuli, and may somewhat be deceived. To achieve this, the actor will emulate some indistinguishable combination of vocal stimuli factors. However, even in doing so, the individual components will not be captured correctly. 
To explain this point, we take the help of an Oliver Sacks case study ``The President's Speech'' \cite{sacks1985president} in which  there are two types of patients: \emph{aphasic}, and \emph{tonal agnostic}. \emph{Aphasic} patients are highly sensitive to expression and tone, and focus on the expressiveness of the emotion to capture it. On the other hand, \emph{tonal agnostic} patients lack any sense of expression and tone, and pay attention to exactness of words and word use to capture the emotion. Neither of these patients can grasp the totality of the natural emotion. However, unlike normal people, these patients, both aphasic and tonal agnostic, can not be lied to or deceived as they have the ability to focus on certain individual factors of emotion which can not be substituted for factors in natural emotion. 

% IT GOES SOUTH FROM HERE.  THE STUFF BELOW HAS NO RELATION TO THE STUFF ABOVE


% In some sense, our NAO model is a test for real versus acted emotions. 
% The question then is whether the observer is able to tell apart natural emotions from acted emotions based on some of the features of the vocal stimuli.
% in which case the test passes, else the test fails. 
% If the test fails, that would mean natural emotions \emph{can} be emulated, and that acted emotions can be used as proxies for natural emotions. If the test passes, however, that would signal towards dichotomy between acted and natural emotions, leading to a low validity and value in using acted stimuli.

% Therefore, in this study, we try to model the observer in the NAO model. The focus is on what part of the vocal stimuli does the observer \emph{attend} to in order to determine the vocal emotion. 
These factors are a result of physiological and psychological changes in the speaker such as the heart rate, breathing rate, muscle tension, and mood. The physiological changes manifest in the voice by changing the spectro-temporal structure of individual sounds \cite{johnstone1999effects, scherer1977cue}. For example, \cite{williams1972emotions, myers2013inherent} argue that vowels and consonants produced in \emph{fear} are often more precisely articulated than they are in \emph{neutral} situations. The physiological changes along with the psychological factors also define the choice of phonemes (i.e. the lexical content). As an example, words of aggressive nature are more likely to be used by an individual in an aggressive mood \cite{whissell1999phonosymbolism}. 
Following this, we determine two basic factors of emotion, \emph{choice of phonemes} and their \emph{manner of delivery}, which we call the \emph{phonetic bases of vocal emotions}. 

% we investigate the phonetic bases of vocal emotions. We define phonetic bases as the \emph{choice of phonemes} and their \emph{manner of delivery}. These phonetic bases are a result of 
Our hypothesis is that these phonetic bases are different in natural and acted emotions.
To test our hypothesis, we train a neural network model for emotion classification tasks on two datasets using \emph{attention} mechanism. The attention aims to capture the phonetic bases of an utterance in order to classify for emotion. We quantify the most \emph{attentive} phonemes under two datasets and compare them across the emotions.

% Unlike a traditional lab setting with controlled variables, we conduct an uncontrolled post-hoc analyses over two existing databases with different speakers and content. To ensure that our analyses have no confounding variables, we, therefore, conduct experimental validation tests to control for any speaker and content-specific biases in databases. 

% \vspace{-1em}


% The communication of vocal emotions which is primarily a combination of an encoding and a decoding process, can be elaborated through the NAO model. The subject {\em expressing} the emotion encodes their emotional state into the low-dimensional speech signal. The subject {\em perceiving} the signal decodes it to make inferences about the state of being of the speaker. We will distinguish between two types of encoders:  the {\em non-actor} who actually experiences the emotion, and the {\em actor} who may not. In all cases, the decoder is an {\em observer}, who's only cue in terms of vocal emotions is the vocal stimuli. The job of the \emph{actor} here is to emulate the natural emotions (of the non-actors) such that the observer is not able to differentiate between natural and acted stimuli, and may somewhat be deceived. 

